A Framework for Studying a Quantum Critical Metal in the Limit $N_f\rightarrow0$

We study a model in 1+2 dimensions composed of a spherical Fermi surface of $N_f$ flavors of fermions coupled to a massless scalar. We present a framework to non-perturbatively calculate general fermion $n$-point functions of this theory in the limit $N_f\rightarrow0$ followed by $k_F\rightarrow\infty$ where $k_F$ sets both the size and curvature of the Fermi surface. Using this framework we calculate the zero-temperature fermion density-density correlation function in real space and find an exponential decay of Friedel oscillations.

==> ZUtilities.tex <==

%%%%common packages%%%%%%
\usepackage{graphicx}
\usepackage{subfigmat}

\usepackage{pgfplots}
\pgfplotsset{compat=1.3}
\usetikzlibrary{arrows.meta}
\usepgfplotslibrary{fillbetween}

%%%%chemistry
\newcommand*\chem[1]{\ensuremath{\mathrm{#1}}}

%%%%some math stuff%%%%%
%sets
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\CC}{\ensuremath{\mathbb{C}}}
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\NN}{\ensuremath{\mathbb{N}}}

%operators
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\tr}{tr}
\newcommand{\re}{\operatorname{Re}}
\newcommand{\im}{\operatorname{Im}}

%symbols
\renewcommand{\d}{\ensuremath{\mathrm{d}}}
\newcommand{\e}{\ensuremath{\mathrm{e}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
